Worksharing Tasks: An Efficient Way to Exploit Irregular and Fine-Grained Loop Parallelism

Shared memory programming models usually provide worksharing and task constructs. The former relies on the efficient fork-join execution model to exploit structured parallelism; while the latter relies on fine-grained synchronization among tasks and a flexible data-flow execution model to exploit dynamic, irregular, and nested parallelism. On applications that show both structured and unstructured parallelism, both worksharing and task constructs can be combined. However, it is difficult to mix both execution models without penalizing the data-flow execution model. Hence, on many applications structured parallelism is also exploited using tasks to leverage the full benefits of a pure data-flow execution model. However, task creation and management might introduce a non-negligible overhead that prevents the efficient exploitation of fine-grained structured parallelism, especially on many-core processors. In this work, we propose worksharing tasks. These are tasks that internally leverage worksharing techniques to exploit fine-grained structured loop-based parallelism. The evaluation shows promising results on several benchmarks and platforms.

==> text/reviews.tex <==
\newcommand{\comment}[2]{\noindent \textbf{Comment #1}: \textsl{#2}}
\newcommand{\question}[2]{\noindent \textbf{Question #1}: \textsl{#2}}
\newcommand{\reply}[1]{\noindent \textbf{Response}: #1}

\subsection{\textbf{Reviewer 1}}
\comment{1}{
    The main issue of this work is the method shows enough implementation 
    improvement and flexible programming, but the novelty is not enough. The 
    authors should address how they could adapt their current method as a 
    general way to provide a stable performance without limitation of 
    scheduling, data structure, algorithm, and hardware. Now, it shows the 
    problem size tuning analysis, how about the other factor during using 
    worksharing task. The strength and impact of this work would be greatly 
    improved.
}
\reply{
    We thank the reviewer for its thorough analysis. In response to this first 
    comment, we would like to highlight that granularity tuning is something 
    inherent to task programming, not something we are adding. In fact, we 
    are providing a mechanism that provides a wider range of granularities that 
    can deliver reasonable performance so that the granularity choice is not so 
    critical as now. This can be seen in Section~\ref{subsec:granularity}. Apart
    from that, in Section~\ref{subsec:strong-scaling} we prove that our solution 
    performs well in two different platforms. Finally, across the whole 
    Section~\ref{sec:evaluation} we show how we are able to get benefit in 
    different algorithms. However, thanks to the reviewer, we found out this was 
    not completely clear and we have rewritten some parts in 
    Section~\ref{sec:background}, \ref{subsec:granularity} and 
    \ref{subsec:strong-scaling}.
}

\comment{2}{
    Additionally, the experimental evaluation section primarily presents the 
    results for 2 different platforms. It would be helpful to show how the 
    proposed worksharing tasks affect the scalability in more different 
    platforms with more data input.
}
\reply{
    For this second round of revision, in order to provide additional experimental 
    evaluation, we have added a new experiment where we compare the performance 
    of region dependences combined with common tasks and with worksharing tasks. 
    This can be seen in Figure~\ref{fig:regions}.
    
    Apart from that, we also added two new series (OMP\_F(D) and OMP\_F(G)) to 
    the granularity evaluation in many-core architecture 
    (Section~\ref{subsec:granularity}), as well as to the strong scaling 
    evaluation (Section~\ref{subsec:strong-scaling}. Those new series can be 
    seen in Figures ~\ref{fig:nbody_granularity}, 
    \ref{fig:stream_granularity}, \ref{fig:strong_scaling_nbody},
    \ref{fig:strong_scaling_matmul}, \ref{fig:strong_scaling_stream} and 
    \ref{fig:strong_scaling_hpccg}.

    Regarding adding more different platforms, we would like to add more 
    platforms but this is unfeasible because of space limitations. However, we 
    expect similar behavior in other platforms. The two platforms we already 
    evaluated are quite different and the benefits from our mechanism showed up 
    in both of them.
}

\comment{3}{
    This work shows a good combination analysis and implementation about how to 
    tuning based on the granularity of problem size per node. The analysis is 
    clear and enough, but it does not show too many new things.
}
\reply{
    Thanks to this comment, we realized that our contribution was not as clear 
    as we thought. We are not only providing an analysis and implementation 
    about how to tuning based on the granularity. We are also providing a novel 
    mechanism that is able to deliver good performance when granularity prevents 
    traditional mechanisms to do so, as it can be shown in \ref{sec:evaluation}.

    For clarifying our contribution, we have added Section~\ref{subsec:utility}.  
}
\subsection{\textbf{Reviewer 2}}
\question{1}{
    Does Fig 1. correspond to any actual or synthetic benchmark? If yes, specify
    the name of the benchmark. If not, I suggest using an actual or even a 
    synthetic benchmark.
}
\reply{
    The original was not corresponding to any actual nor synthetic benchmark. 
    According to this suggestion, we have replaced the previous chart from a new 
    one that actually corresponds to a synthetic benchmark. The code of the 
    benchmark have been added in Code~\ref{lst:synthetic}. Accordingly, we have 
    updated the description of the chart in Section~\ref{sec:background}.
}

\question{2}{
    VI. E: "For all the versions, we have selected the best configuration of 
    block size, chunk size, and number of workers, if applicable". How did you 
    find the best configuration? What was the search space?
}
\reply{
    We performed an analysis of each of the parameters to find the best overall 
    configuration. As this was not clear, we have added a clarifying sentence 
    in Section~\ref{subsec:strong-scaling}.

    With regard to the search space, the methodology we used is following.
    Regarding the block size, we start from the biggest TS which 
    is when TS=PS (creating just one task). Then we decrement it until a point 
    where either the performance does not vary anymore between hops, or the 
    peformance is so low that the execution hardly finishes in a reasonable 
    time. With respect to the chunk size, we follow similar methodology. We 
    start from the biggest CS which is when CS=TS (just one chunk per block). 
    Then we decrement until the a point where either the CS is 1 or the 
    performance is so low that the execution hardly finishes in a reasonable 
    time. With regard to the number of workers, we never go beyond the NUMA 
    node---this is the upper bound. Then, we decrement until N=2. N=1 does not 
    make sense since as it is like using a task. 
}

\question{3}{
    As you have pointed out, parameters like chunk size affect performance. (I)
    What is the performance of each approach (for all experiments) with default 
    parameters? (II) What would be a reasonable way to choose chunk size for 
    your approach (other than exhaustive search and auto-tuning)?
}
\reply{
    Worksharings with static scheduler are usually the best option with default 
    parameters. They introduce very few overhead and they are able to 
    automatically set a chunksize that gives work to all the threads. In 
    contrast, any task-based implementation must be manually blocked, and so, 
    the granularity must be explicitly tuned, so there is no "default parameter" 
    for this. When comparing task versions (assuming granularity has been tuned) 
    to worksharing tasks (with default chunksize and number of collaborators) 
    they usually perform similar if there is enough problem size per core. 
    Otherwise, worksharing tasks perform better than common tasks.

    We recommend choosing a chunksize that permits each collaborator having at 
    least one chunk to execute. In general, CS=TS/N, should be a good value. 
    However, depending on other parameters as well as the application, this 
    will not always be the best option. For instance, if the task is already 
    fine-grained, chunks will become too small if we do CS=TS/N. Also, another 
    factor to consider is the cost of the computation. Heavier computations will 
    perform well with smaller chunksizes than lighter computations. We have 
    added this conclusions at the end of Section~\ref{subsec:cs-granularity}. 
}

\comment{1}{
    OMP\_F (code 3) version is used in many comparisons. However, the "dynamic" 
    and "guided" versions of this are not presented in the evaluation. For 
    completeness, this comparison should also be included (even if their 
    performance is worse than OMP\_F).
}
\reply{
    As the reviewer points out, dynamic and guided versions were not presented 
    in the evaluation. We thought static scheduler was the best option as it is 
    introducing fewer overhead than the others and the applications presented 
    are not specially imbalanced. However, it is right that for completeness, 
    they should be included and we did it in
    Figures~\ref{fig:nbody_granularity}, \ref{fig:stream_granularity}, 
    \ref{fig:strong_scaling_nbody}, \ref{fig:strong_scaling_matmul}, 
    \ref{fig:strong_scaling_stream} and \ref{fig:strong_scaling_hpccg}.

    We also updated the discussions of those charts in 
    Section~\ref{sec:evaluation} to include considerations about the new 
    versions included, as well as a brief introduction to them in 
    Section~\ref{subsec:benchmarks}.
}

\comment{2}{
    Add additional experiments mentioned in the comments.
}
\reply{
    We added the dynamic and guided versions of OMP\_F to the granularity and 
    strong scaling experiments, as requested by the reviewer in the previous 
    comment. Please, see reply of previous comment for details.
}

\comment{3}{
    Add more benchmarks (at least in text) which could benefit from this 
    approach.
}
\reply{
    All the benchmarks that currently use OpenMP worksharings (i.e. omp for), 
    could actually use our approach. The applicabilty of our mechanism is as 
    broad as OpenMP worksharings applicability. The only requirement is that 
    iterations of the loop must be independent. Then, for getting benefit from 
    our approach, they should be in an scenario where problem size per core is 
    insufficient to actually exploit all the resources without incurring in so 
    much overhead. This happens frequently in strong scaling experiments where 
    the problem size is fixed and the resources augment, consequently reducing 
    the problem size per node until either not having enough parallelism or 
    incurring in overheads because of too fine-grained block sizes.

    We have added Section~\ref{subsec:applicability} to summarize this. There, 
    we also enumerate some benchmarks where we expect to get benefit from 
    worksharing tasks.
}
\subsection{\textbf{Reviewer 3}}
\comment{1}{
    The way that concepts (such as "worksharing", "fork-join execution", 
    "structured parallelism", "task-based programming") are used in this paper 
    makes the arguments confusing. The authors mentioned OpenMP is fork-join 
    based and structured. But OpenMP also supports the concept of "task". On 
    the other hand, the authors did not mention any actual library for 
    task-based programming. I assume the authors refer to Cilk-style programming.
}
\reply{
    We have added some examples of task-based programming in 
    Section~\ref{sec:intro}. 
}

\comment{2}{
    The term "worksharing" is not commonly used to represent loop-based 
    parallelism. It might be better to use "structured" (vs "unstructured") 
    or "regular" (vs "irregular"). Similarly, the concept of "worksharing task" 
    is not intuitively clear.
}
\reply{
    Actually, worksharing refers to a mechanism/technique while 
    structured/unstructured (or regular/irregular) refer to an application 
    pattern. Worksharing technique can actually be used to deal either with 
    regular or irregular parallelism. However, it usually does not perform well 
    when dealing with irregular/unstructured patterns due to its rigid 
    synchronization.

    Regarding the concept of "worksharing task", it is the best name we were 
    able to find, since it is like a task in almost everything, but it does 
    share its work among several threads instead of being run by a single one.
}

\comment{3}{
    The contribution/novelty of the "worksharing task" is unclear. The latest 
    OpenMP also supports both static and dynamic task generation and Cilk, on 
    the other hand, also supports loop-level parallelization.
}
\reply{
    Although we do not really know what the reviewer means with static/dynamic 
    task generation, we can guarantee that our mechanism is not present in 
    OpenMP. We have thoroughly evaluated the OpenMP standard, as well as 
    discussed about this topic with some OpenMP Board commitee members and there 
    is nothing in OpenMP like worksharing tasks. 

    Regarding Cilk loop-level parallelization, the cilk\_for contains an 
    implicit cilk\_sync at the end of every loop iteration. This makes it more 
    similar to OpenMP worksharings, with a rigid synchronization. To clarify these
    points, we have added new content in Section~\ref{subsec:utility} 
    outlining the main contributions of worksharing tasks.
}

\comment{4}{
    In the motivation part, the authors mention that loop-based parallelism 
    works better for machines with a small number of cores and task-based 
    parallelism works better when there are many cores. This argument does not 
    makes sense.
}
\reply{
    Worksharing technique implies a very rigid synchronization scheme. In general, whenever 
    a thread finishes its own work, it must wait until all the rest also 
    finishes to leave that team and get new work. As the number of cores grow, 
    it becomes easier to find load imbalance, and so, a lot of cpu time is 
    wasted just waiting for the last thread to finish. In contrast, task 
    programming allows a data-flow execution. Thus, synchronization is more 
    fine-grained, and threads can move forward when the data is ready, instead of 
    waiting just because a thread of its team still had not finished. 
}

\comment{5}{
    For Fig. 1, the authors discuss task granularity and phases, without 
    mentioning anything about the application.
}
\reply{
    Actually, the previous Fig. 1 was a theoretical chart, and the phases we 
    discussed about in the text where chart phases, not application ones. 
    However, we have seen that the previous Fig. 1 and its discussion was 
    causing some doubts between the reviewers. Therefore, we replaced the 
    previous Fig. 1 and part of its discussion. Now, it is based on a synthetic 
    benchmark (the code has been included in the paper) and we clarify that 
    we discuss about chart phases rather than application phases.
}

\comment{6}{
    The motivation section does not effectively motivate this work. The tradeoff 
    between task grnaularity and performance gains is well-known.
}
\reply{
    We have realized that the motivation was not completely clear, as the 
    reviewer points out. There are three main points that motivate our work.
    The starting point is that developers want to use task-based parallelism to 
    deal with fine-grain loop parallelism because of the key benefits tasks 
    provide. However, task programming have some difficulties/problems that 
    threaten their use. The first one is that granularity is critical. Thus, 
    developers must perform a granularity analysis to choose a good one. However, 
    and this is the second problem, not always exists a good granularity. 
    Finally, runtimes cannot develop sophisticated task management policies 
    because when dealing with large number of tasks, those could impact the 
    performance. 

    Given these problems/difficulties, we state that an effort must be done to 
    mitigate/solve them, and encourage users to use task-based parallelism 
    rather than loop-based.

    We have added new text at the end of Section~\ref{sec:background} to clarify 
    this.
}

\question{1}{
    As Fig. 2 shows, assigning chunks to different workers in fact introduces 
    some overhead, especially when the chunk size is small, which may cause 
    too many requests to the scheduler. So how to determine the minimum chunk 
    size, or, the maximum number of chunks for a task, to avoid the overhead?
}
\reply{
    We recommend choosing a chunksize that permits each collaborator having at 
    least one chunk to execute. So, CS=TS/N, should be a good value usually. 
    However, depending on other parameters as well as the application, this 
    will not always be the best option. For instance, if the task is already 
    fine-grained, chunks will become too small if we do CS=TS/N. Also, another 
    factor to consider is the cost of the computation. Heavier computations will 
    perform well with smaller chunksizes than lighter computations. We have 
    added this conclusions at the end of Section~\ref{subsec:cs-granularity}. 
}

\question{2}{
    As mentioned in the paper, the number of collaborators (N) is critical to 
    achieving good performance when using work sharing tasks, but determining N 
    seems challenging. Is there any solution to decide the optimal N for the 
    tasks in a given application?
}
\reply{
    The number of collaborators (N) is actually important for achieving good 
    performance. There are some considerations for choosing it. Firstly, the 
    user must generate at least one worksharing task per team, ideally more. The 
    same happens when using common tasks: at least one task per core, ideally 
    more, to prevent them from becoming idle. Therefore, if we have many tasks, 
    we can use smaller teams. Oppositely, if we have only few tasks, we should 
    use bigger teams. Secondly, the collaborators inside a team will fight for 
    getting the team lock. Thus, contention increments. So, it is not a good 
    idea using just one group with all the cores available. Finally, we do not 
    recommend going beyond a CPU socket when setting up teams. So, if a socket, 
    for instance, contains 24 CPUs, do not use teams bigger than 24. As a 
    general recommendation, we suggest using one or two teams per socket. Our 
    default value is one team per socket. 

    This has been added in Section~\ref{subsec:granularity}.
}

\question{3}{
    In strong scaling experiments, the best configurations need to be applied 
    for all the versions. Are the best configurations determined by enumerating 
    all the setting combinations?
}
\reply{
    We performed an analysis of each of the parameters to find the best overall 
    configuration. As this was not clear, we have added the previous sentence 
    in Section~\ref{subsec:strong-scaling}.
}

\question{4}{
    In the left chart of Fig. 5, the OpenMP behaves much better, especially for 
    OMP\_T+F16 with small chunk size. The paper explains these results as "the 
    policy just uses the chunk size as a minimum and may assign bigger chunks 
    to thread if chunksize is too small". But if that is the case, why does 
    changing the chunksize from 32 to 64 make performance better for OMP\_T+F16?
}
\reply{
    A key point of this chart is that each series cannot compare with the rest. 
    It can only be compared with other points within the same series. The 
    reason for that is that each series is using different parameters. We have 
    added a sentence clarifying this fact in Section~\ref{subsec:cs-granularity}.

    Regarding the second part of the question, guided scheduling is a dynamic 
    scheduling policy that assigns iterations to threads in chunks. The size of 
    the chunks is proportional to the number of unassigned chunks divided by the 
    number of threads in the team, with the restriction that the chunk size can 
    never be lower than the value indicated by the user. So, the guided policy 
    usually starts with big chunks and then starts reducing the chunk size to 
    keep load balance among the different threads. So, at the end, when 
    assigning the last chunks, the difference pops up, because in that part the 
    user value does actually make a difference, although not much.

    We have rewritten our explanation about this in 
    Section~\ref{subsec:cs-granularity}.
}

\subsection{\textbf{Reviewer 4}}
\question{1}{
    The authors precise that the new construct "accepts" the chunksize clause. 
    If it is not mandatory, what is its default setting (which, as the authors 
    demonstrate, is critical)?
}
\reply{
    The default chunksize is TS/N so that each collaborator can have at least 
    one chunk for running. This information has been added in 
    Section~\ref{subsec:syntax}.
}
\comment{1}{
    I guess the worksharing task workers are launched in the same way as tasks, 
    which is not quite predictable, but the best chunk size for each worksharing 
    task will depend on how the workers are launched, hence finding he best 
    setting is not possible.
}
\reply{
    Worksharing task workers are launched dynamically, and so it is not quite 
    predictable as the reviewer points out. However, we have added several 
    considerations and a suggestion for finding the best chunk size in 
    Section~\ref{subsec:cs-granularity}.
}

\question{2}{
    The annotation seems particularly useful for imbalanced applications. 
    However, in the benchmarks the applications such as Matmul or N-body does 
    not seem inherently imbalanced. Could the authors elaborate why do we see 
    such an improvement over regular "omp for" for big datasets in your strong 
    scaling experiment?
}
\reply{
    We have thoroughly reviewed the charts presenting Matmul and N-body results 
    for the strong scaling experiment. Unfortunately, we are not able to see any 
    significant improvement over regular "omp for" for big datasets. Actually, 
    the improvements for those benchmarks are for the lowest datasets. The 
    reason for the improvements in those scenarios is that "omp for" suffers 
    lack of parallelism, while worksharing tasks does not.
}

\question{3}{
    The authors use a NUMA architecture in the first setup, where non NUMA aware 
    omp-for or task-for loops may loose performance. The authors do not talk 
    about the location and size of the worker team other than "close in the 
    physical layout" and seem to use 2 teams? How does this affect the 
    performance of this technique?
}
\reply{
    Regarding the first question, for the strong scaling experiment, different
    sizes of the team has been used. This is because we have always used the 
    best setup which is not the same for all the scenarios. Being that said, we 
    can guarantee that the team is always within a NUMA node. This is one of the 
    advices we introduced in Section~\ref{subsec:granularity}.

    With respect to the second question, all the experiments have been run using 
    the interleaving policy offered by the numactl command. Hence, the data has 
    been evenly spreaded among the NUMA nodes. That way, NUMA effects should be 
    minimized and not make any significant difference.

    New content regarding this has been added to Section~\ref{subsec:env}.
}

\comment{2}{
    Providing the worksharing tasks code corresponding to Fig. 2 (top) would be
    helpful.
}
\reply{
    Code~\ref{lst:pipelining} has been added in Section~\ref{subsec:syntax} 
    replacing the simple C/C++ exmaple.
}

\comment{3}{
    The related work section is essentially about OpenMP, I would suggest to 
    separate OpenMP and wider related work.
}
\reply{
    We have separated the related work into OpenMP related work and Non-OpenMP 
    related work. Also, we have added a review of Cilk loop-level 
    parallelization (cilk\_for).
}

\question{4}{
    I would be curious to know how Code 3+dynamic/guided and Code 
    6+static/dynamic behave. Are they pertinent?
}
\reply{
    We have added Code 3+dynamic/guided schedulers to our granularity and 
    strong scaling experiments. Concretely, they have been added in Figures 
    \ref{fig:nbody_granularity}, \ref{fig:stream_granularity}, 
    \ref{fig:strong_scaling_nbody}, \ref{fig:strong_scaling_matmul}, 
    \ref{fig:strong_scaling_stream} and \ref{fig:strong_scaling_hpccg}.

    We also updated the discussions of those charts in 
    Section~\ref{sec:evaluation} to include considerations about the new 
    versions included, as well as a brief introduction to them in 
    Section~\ref{subsec:benchmarks}.

    Regarding Code 6+static/dynamic, what we tried to do in Code 6 is to 
    replicate as much as possible the behavior of worksharing tasks using 
    available mechanisms in OpenMP. Thus, we chose guided scheduler since we 
    think it is the one that replicates better the behavior. Apart from that, 
    after adding OMP\_F(D) and OMP\_F(G), the charts already contain many series 
    so adding more may hinder its visualization.
}
\subsection{\textbf{Metareview}}
\comment{1}{
    The use of terminology in a confusing manner.
}
\reply{
    We have clarified the use of terminology on those parts where it was not 
    clear. As well, we have provided appropriate rebuttal, along with an 
    explanation of why we consider the terminology is properly used for the 
    other cases where we consider it has been used right. Please, see replies 
    to comments 1 and 2 from Reviewer 3 to further details.
}

\comment{2}{
    Lack of sufficient comparative evaluation.
}
\reply{
    We have added Figure~\ref{fig:regions} comparing the performance of using 
    region dependences with common tasks and with worksharing tasks. 
    
    Additionally, we have added two new series (OMP\_F(D) and OMP\_F(G)) to the 
    granularity evaluation in many-core architecture 
    (Section~\ref{subsec:granularity}) as well as to the strong scaling 
    evaluation (Section~\ref{subsec:strong-scaling}. See Figures~\ref{fig:nbody_granularity}, 
    \ref{fig:stream_granularity}, \ref{fig:strong_scaling_nbody},
    \ref{fig:strong_scaling_matmul}, \ref{fig:strong_scaling_stream} and 
    \ref{fig:strong_scaling_hpccg}.
}

\comment{3}{
    Lack of detailed discussion of the experimental setup to enable 
    reproducibility.
}
\reply{
    We have added all the parameters to each of the charts in order to enable 
    reproducibility of the experiments. It is possible to see those parameters 
    in Figures~\ref{fig:nbody_granularity}, \ref{fig:stream_granularity},
    \ref{fig:cs_granularity}, \ref{fig:strong_scaling_nbody}, 
    \ref{fig:strong_scaling_matmul}, \ref{fig:strong_scaling_stream} and 
    \ref{fig:strong_scaling_hpccg}.
}

\comment{4}{
    Insufficient choice of benchmarks that can benefit from this approach, and 
    limited justification for why such benchmarks can benefit.
}
\reply{
    Although we would like to do so, we cannot add new benchmarks to the 
    experimentation due to space constraints. However, as suggested by 
    Reviewer 2, we have added some benchmarks in text that can benefit from 
    this approach, and the corresponding explanation of why. This can be found 
    in Section~\ref{subsec:applicability}. Please, see reply to comment 3 from 
    Reviewer 2 for further details.
}

